DNS: Determinantal Point Process Based Neural Network Sampler for Ensemble Reinforcement Learning

Application of ensemble of neural networks is becoming an imminent tool for advancing the state-of-the-art in deep reinforcement learning algorithms. However, training these large numbers of neural networks in the ensemble has an exceedingly high computation cost which may become a hindrance in training large-scale systems. In this paper, we propose DNS: a Determinantal Point Process based Neural Network Sampler that specifically uses k-dpp to sample a subset of neural networks for backpropagation at every training step thus significantly reducing the training time and computation cost. We integrated DNS in REDQ for continuous control tasks and evaluated on MuJoCo environments. Our experiments show that DNS augmented REDQ outperforms baseline REDQ in terms of average cumulative reward and achieves this using less than 50% computation when measured in FLOPS.

==> DPP.tex <==


% \subsection{Definitions}
% \begin{definition}
% Let $L$: $\mathcal{S}^2\rightarrow\mathbb{C}$ be Hermitian, positive semi-definite. An $L$-ensemble is a determinantal point process $\boldsymbol{X}$ on $\mathcal{S}$ with kernel $K:=I-(I+L)^{-1}$ and distribution
% \begin{equation}
% \label{eqn:l-ensemble}
% P(\boldsymbol{X}=x)=det(L_x)det(I+L)^{-1}
% \end{equation}
% for any $x\subset\mathcal{S}$, where $L_x$ is the submatrix of $L$ indexed by $x\times x$.
% \end{definition}
% \renewcommand\thetheorem{1}
% \begin{lemma}
% Let $D$ be an $N\times N$ diagonal matrix and let $M$ be an arbitrary $N\times N$ matrix. The determinant of $(D + M)$ is :
% \begin{equation}
% det(D+M) = \sum_{S\subseteq\mathcal{S}}det(D_S)det(M_S).
% \end{equation}
% \end{lemma}
% The proof of Lemma 1 can be found in \citep{Collings-1983-TAS}.

% From Lemma 1, (\ref{eqn:l-ensemble}) can be re-written as:
% \begin{equation}
% P(\boldsymbol{X}=x)=det(L_x)(\sum_{x\subseteq\mathcal{S}}det(L_x))^{-1}
% \end{equation}
% and is thus normalized.
% \paragraph{Remarks.}
% \begin{enumerate}[i.]
% \item While (\ref{eqn:K}) gives the probability that a set is contained in the DPP, (\ref{eqn:l-ensemble}) gives the exact probability that a sampled set is from the DPP and is thus more relevant for set selection tasks requiring samples from different regions in a feature space since more diverse sets have higher probability and are thus more likely to be selected. 
% \item Since $L$ is Hermitian positive semi-definite, $K$ is also Hermitian positive semi-definite.
% \item There is no requirement that all eigenvalues of $L\,$are are less than or equal to 1.
% \end{enumerate}

% In many machine learning applications $L$ is a symmetric matrix (hence Hermitian) that is constructed using a raw data feature matrix $\boldsymbol{A}$, i.e $L=\boldsymbol{AA}^{\boldsymbol{T}}$ which is positive semi-definite. In this work the centered kernel alignment (CKA) index$\,$was calculated as a measure of the similarity of $N$ target network activation matrices and these indices were used as entries of the similarity matrix $L$ $\in\mathbb{R}^{^{N\times N}}$:
% \[
% L_{ij}=CKA(x_i,x_j)\in[0,1], i\in\{1,\ldots,N\}.
% \]
% Other choices for $L$ include matrices based on pairwise similarities between points , e.g. based on a distance criterion.$\,$Since not all similarity matrices are positive semi-definite, $L\,$can be approximated with the closest positive semi-definite such that the relative similarity strengths among point pairs are preserved. 


% \begin{proposition}
% The nearest positive semi-definite matrix to a symmetric matrix to
% $L\in\mathbb{R}^{^{N\times N}}$ is a diagonal perturbation of $L$:
% \[
% \overset{\sim}{L}=L+D,
% \]
% where $D=diag((\lambda_i+|\lambda_i|)/2)$, and
% $\lambda_i, i\in\{1,\ldots,N\}$ are eigenvalues from the spectral
% decomposition of $L$.

% \end{proposition}

% \begin{proof}
% The nearest positive semi-definite matrix $\overset{\sim}{L}$ to a matrix $L$ can be computed via a spectral decomposition of $B=(L+L^T)/2=\boldsymbol{V}\Lambda\boldsymbol{V}^T=\boldsymbol{V}diag(\lambda_i)\boldsymbol{V}^T$ as:
% \[
% \overset{\sim}{L}=\boldsymbol{V}diag(d_i)\boldsymbol{V}^T,\]
% where
% \[d_i=
% \begin{cases}
% \lambda_i,&\lambda_i\geq 0\\
% 0,&\lambda_i<0
% \end{cases}
% \]
% or equivalently as: 
% \begin{equation}
% \label{eqn:psd}
% \overset{\sim}{L}=(B+H)/2,
% \end{equation}
% where $H=\boldsymbol{V}diag(|\lambda_i|)\boldsymbol{V}^T$\citep{higham-1988-LAA}.
% Since $L$ is symmetric, $B=L=\boldsymbol{V}diag(\lambda_i)\boldsymbol{V}^T$ and
% $H=\boldsymbol{V}diag(|\lambda_i|)\boldsymbol{V}^T.$ It follows from (\ref{eqn:psd}) that $\overset{\sim}{L}=L+D$ where $D=(diag(\lambda_i)+diag(|\lambda_i|))/2=diag((\lambda_i+|\lambda_i|)/2)$.
% \end{proof}

% \begin{definition}
% A $k$-DPP on discrete set $\mathcal{S}$ is a distribution over all subsets of $\mathcal{S}$ with cardinality k and is thus a conditioning of a standard DPP on the event that a subset $X$ of $\mathcal{S}$ has a fixed size. A k-DPP thus gives probabilities
% \begin{equation}
% P^{\boldsymbol{(k)}}(\boldsymbol{X}=x)=det(L_x)(\sum_{\substack{x
% \subseteq\mathcal{S}\\|x|=k}}det(L_x))^{-1},
% \end{equation}
% where $|x|=k$ and $L$ is a positive semi-definite kernel.\citep{Kulesza-2011-ICML}
% \end{definition}
% Because $k$-DPPs only model contents of a set, they are less costly than
% standard DPPs and are useful in situations where sample size is constrained,
% for example by empirical bounds or hardware restrictions \citep{Zhang-2017-AUI}.

% \begin{theorem}
% \end{theorem}

